Isomorphism Is Not Enough: An Agentic Audit of Verified Code Generation in Lean

Agentic systems have recently emerged as state-of-the-art approaches for automated theorem proving in formal mathematics. To assess how far these capabilities extend to program verification and how reliably existing benchmarks can measure them, we audit CLEVER, a Lean 4 benchmark for verifiable code generation, using three independent agentic stacks based on Claude Opus 4.6, GPT-5.4, and Kimi K2.5. Our audit finds arguably erroneous reference specifications in 80 of 161 entries, each accepted by the benchmark's authors, distills a taxonomy of benchmark errors, and exposes structural limitations of isomorphism-based scoring, whose signal breaks down when generated and reference specifications formalize different yet defensible readings. In the process, the stacks generate arguably valid specifications for up to 98.8% of entries, certify implementations against sound reference specifications for up to 92.3%, and reach up to 96.2% end-to-end success over entries with sound premises, suggesting that CLEVER no longer stresses modern agentic provers as much as its design intended. Looking ahead, we translate our findings into recommendations for future work, with our error analysis doubling as a repair list for CLEVER and a heuristic checklist for the next generation of benchmarks.

==> floats/claude_flags_impl.tex <==
\mainfloatbegin
  \centering
  \moveups
  \includegraphics[width=\textwidth]{images/sankey_impl_claude.png}
  \moveup
  \moveup
  \moveups
  \caption{Distribution of Claude's output flags for \proofgen{} against the reference and against its simple and guided generated specifications, in the color scheme of Figure~\ref{fig:claude-flags}. The color of a specification \flagISSUE{} follows its source: reference in the first row, generated in the others.}
  \moveup
  \moveup
  \moveups
  \label{fig:claude-flags-impl}
\mainfloatend


==> floats/claude_flags_spec.tex <==
\mainfloatbegin
  \centering
  \moveups
  \includegraphics[width=\textwidth]{images/sankey_spec_claude.png}
  \moveup
  \moveup
  \moveups
  \caption{Distribution of Claude's output flags for the \speciso{} runs. The color scheme, used throughout the paper, is green for \flagOK{}, red for \flagFAIL{}, yellow for \flagMISMATCH{}, blue for \flagISSUE{} in benchmark components, orange for \flagISSUE{} in generated components, and purple for issues in both. The hatched segment of the Multiple specifications row marks the 56 entries already \flagOK{} in the guided run, which were not re-tested.}
  \moveup
  \moveup
  \moveups
  \label{fig:claude-flags}
\mainfloatend


==> floats/floatspots.tex <==
\makeatletter
\newif\ifshowfloatspots
\newcommand{\floatspot}[1]{%
  \ifshowfloatspots\par\noindent{\tiny\ttfamily\color{red}[#1]}\par\fi
  \@ifundefined{floatspot@#1}{}{\@nameuse{floatspot@#1}}}
\newcommand{\putfloat}[4]{%
  \@ifundefined{floatspot@#1}{\@namedef{floatspot@#1}{}}{}%
  \expandafter\g@addto@macro\csname floatspot@#1\endcsname{%
    \def\floatenv{#2}\def\floatpos{#3}\input{#4}}}
\newcommand{\mainfloatbegin}{\edef\floatspot@tmp{\noexpand\begin{\floatenv}[\floatpos]}\floatspot@tmp}
\newcommand{\mainfloatend}{\edef\floatspot@tmp{\noexpand\end{\floatenv}}\floatspot@tmp}
\makeatother


==> floats/overview.tex <==
\mainfloatbegin
  \centering
  \resizebox{\textwidth}{!}{\input{images/overview}}
  \caption{Schematic overview of our experimental pipeline. The four generation and proof tasks are identified in yellow: \clever{}'s original intended setup spans horizontally in red across the top row, while other pathways represent our custom variations of the setup. The dashed portion in the top-right corner is the preliminary experimentation setup of Appendix~\ref{app:preliminary-experiments}.}
  \label{fig:overview}
\mainfloatend


==> images/overview.tex <==
\begin{tikzpicture}[x=1pt, y=-1pt, line width=1pt, line cap=butt, line join=miter]
  \definecolor{ovYellow}{HTML}{FFFFCC}
  \definecolor{ovGrey}{HTML}{F5F5F5}
  \definecolor{ovRedFill}{HTML}{F8CECC}
  \definecolor{ovRedLine}{HTML}{B85450}
  \definecolor{ovOrangeFill}{HTML}{FFE6CC}
  \definecolor{ovOrangeLine}{HTML}{D79B00}
  \definecolor{ovGreenFill}{HTML}{D5E8D4}
  \definecolor{ovGreenLine}{HTML}{82B366}
  \definecolor{ovBlueFill}{HTML}{DAE8FC}
  \definecolor{ovBlueLine}{HTML}{6C8EBF}
  \definecolor{ovLabel}{HTML}{333333}
  \pgfdeclarearrow{
    name = ovArrow,
    setup code = {
      \pgfarrowssettipend{1.118pt}
      \pgfarrowssetlineend{-5.25pt}
      \pgfarrowssetbackend{-7.5pt}
      \pgfarrowshullpoint{1.118pt}{0pt}
      \pgfarrowshullpoint{-7.5pt}{4pt}
      \pgfarrowshullpoint{-7.5pt}{-4pt}
    },
    drawing code = {
      \pgfsetdash{}{0pt}\pgfsetmiterjoin
      \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
      \pgfpathlineto{\pgfqpoint{-7pt}{3.5pt}}
      \pgfpathlineto{\pgfqpoint{-5.25pt}{0pt}}
      \pgfpathlineto{\pgfqpoint{-7pt}{-3.5pt}}
      \pgfpathclose
      \pgfusepathqfillstroke
    },
  }
  \newcommand*\ovfont[1]{\fontfamily{ptm}\fontsize{#1}{#1}\selectfont\frenchspacing}
  \tikzset{
    ov column/.style={fill=ovYellow, fill opacity=0.8, draw=none, rounded corners=15pt},
    ov orange/.style={fill=ovOrangeFill, draw=ovOrangeLine},
    ov green/.style={fill=ovGreenFill, draw=ovGreenLine},
    ov blue/.style={fill=ovBlueFill, draw=ovBlueLine},
    ov dashed/.style={dash pattern=on 3pt off 3pt},
    ov edge/.style={draw=black, -ovArrow},
    ov text/.style={anchor=base west, inner sep=0pt, text=black, font=\ovfont{12}},
    ov label/.style={ov text, text=ovLabel, font=\ovfont{10}},
    ov small/.style={ov text, text=ovLabel, font=\ovfont{9}},
    ov arrow/.style={anchor=base, inner sep=0pt, text=ovLabel,
      font=\usefont{U}{pzd}{m}{n}\fontsize{9.4}{10}\selectfont},
  }
  \useasboundingbox (138.937,94.5) rectangle (787.181,348.316);

  \path[ov column] (625,95) rectangle ++(100,252);                %
  \begin{scope}
    \clip (624.5,94.5) rectangle (724.5,150.5);
    \foreach \c in {714.59,745.71,776.82,807.93,839.05,870.16}
      \draw[white, line width=12pt] (\c-80,80) -- (\c-165,165);
  \end{scope}
  \path[ov column] (495,147) rectangle ++(100,200);               %
  \path[ov column] (360,147) rectangle ++(100,200);               %
  \path[ov column, draw=ovGrey, draw opacity=0.8, line width=0.5pt]
    (220,147) rectangle ++(100,200);                              %
  \path[fill=ovRedFill, fill opacity=0.5, draw=ovRedLine, draw opacity=0.5,
    rounded corners=7.5pt] (140,151) rectangle ++(645,50);        %

  \draw[ov edge] (380,176) -- (440,176);
  \draw[ov edge] (380,231) -- (440,231);
  \draw[ov edge] (380,176) -- (390,176) -- (390,206) -- (660,206) -- (660,221) -- (700,221);
  \draw[ov edge] (240,258.5) -- (250,258.5) -- (250,241) -- (300,241);
  \draw[ov orange] (160,156) rectangle ++(80,40);                 %
  \draw[ov orange] (160,228.5) rectangle ++(80,60);               %
  \draw[ov green] (300,156) rectangle ++(80,40);
  \draw[ov green] (300,211) rectangle ++(80,40);
  \draw[ov green] (300,266) rectangle ++(80,20);
  \draw[ov green] (300,286) rectangle ++(80,20);
  \draw[ov green] (300,306) rectangle ++(80,20);
  \draw[ov orange] (360,100) rectangle ++(80,40);                 %
  \draw[ov edge] (240,176) -- (300,176);
  \draw[ov edge] (240,176) -- (260,176) -- (260,231) -- (300,231);
  \draw[ov edge] (240,176) -- (260,176) -- (260,236.5)
    .. controls +(5.85,0) and +(5.85,0) .. (260,245.5) -- (260,296) -- (300,296);
  \draw[ov edge] (240,258.5) -- (250,258.5) -- (250,306) -- (300,306);
  \draw[ov blue] (440,156) rectangle ++(80,40);
  \draw[ov blue] (440,211) rectangle ++(80,40);
  \draw[ov blue] (440,266) rectangle ++(80,20);
  \draw[ov blue] (440,286) rectangle ++(80,20);
  \draw[ov blue] (440,306) rectangle ++(80,20);
  \draw[ov edge] (380,296) -- (440,296);
  \draw[ov green] (570,211) rectangle ++(80,40);
  \draw[ov green] (570,266) rectangle ++(80,40);
  \draw[ov green] (570,156) rectangle ++(80,40);
  \draw[ov orange, ov dashed] (570,100) -| (650,140) -| cycle;   %
  \draw[ov edge] (380,176) -- (390,176) -- (390,206) -- (530,206) -- (530,231) -- (570,231);
  \draw[ov edge] (380,231) -- (390,231) -- (390,258.5) -- (530,258.5) -- (530,286) -- (570,286);
  \draw[ov edge] (400,140) -- (400,144) -- (530,144) -- (530,176) -- (570,176);
  \draw[ov blue, ov dashed] (700,100) -| (780,140) -| cycle;
  \draw[ov blue] (700,156) rectangle ++(80,40);
  \draw[ov blue] (700,211) rectangle ++(80,40);
  \draw[ov blue] (700,266) rectangle ++(80,40);
  \draw[ov edge] (650,231) -- (700,231);
  \draw[ov edge] (380,231) -- (390,231) -- (390,258.5) -- (660,258.5) -- (660,276) -- (700,276);
  \draw[ov edge] (650,286) -- (700,286);
  \draw[ov edge] (400,140) -- (400,144) -- (660,144) -- (660,176) -- (700,176);
  \draw[ov edge] (650,186) -- (700,186);
  \draw[ov edge, ov dashed] (400,140) -- (400,144) -- (660,144) -- (660,130) -- (700,130);
  \draw[ov edge, ov dashed] (650,120) -- (700,120);
  \draw[ov edge] (400,140) -- (400,172) .. controls +(5.197,0) and +(5.197,0) .. (400,180)
    -- (400,186) -- (440,186);
  \draw[ov edge] (400,140) -- (400,172) .. controls +(5.197,0) and +(5.197,0) .. (400,180)
    -- (400,227) .. controls +(5.197,0) and +(5.197,0) .. (400,235)
    -- (400,241) -- (440,241);
  \draw[ov edge] (400,140) -- (400,172) .. controls +(5.197,0) and +(5.197,0) .. (400,180)
    -- (400,227) .. controls +(5.197,0) and +(5.197,0) .. (400,235)
    -- (400,292) .. controls +(5.197,0) and +(5.197,0) .. (400,300)
    -- (400,306) -- (440,306);

  \node[ov text] at (366.05,116.5) {Ground-Truth};
  \node[ov text] at (367.84,131.5) {Specification};
  \node[ov text] at (576.03,116.5) {Ground-Truth};
  \node[ov text] at (571.50,131.5) {Implementation};
  \node[ov text] at (191.50,172.5) {NL};
  \node[ov text] at (171.50,187.5) {Description};
  \node[ov text] at (174.08,248) {Test Cases};
  \node[ov text] at (194.83,262) {\&};
  \node[ov text] at (166.56,277) {NL Examples};
  \foreach \b/\c in {172.5/187.5, 227.5/242.5} {
    \node[ov text] at (314.84,\b) {Generated};
    \node[ov text] at (307.84,\c) {Specification};
    \node[ov text] at (447.83,\b) {Isomorphism};
    \node[ov text] at (466.16,\c) {Proof};
  }
  \foreach \b/\c in {172.5/187.5, 227.5/242.5, 282.5/297.5} {
    \node[ov text] at (584.83,\b) {Generated};
    \node[ov text] at (571.50,\c) {Implementation};
  }
  \foreach \b/\c in {116.5/131.5, 172.5/187.5, 227.5/242.5, 282.5/297.5} {
    \node[ov text] at (711.17,\b) {Correctness};
    \node[ov text] at (726.16,\c) {Proof};
  }
  \node[ov text] at (308.83,279.5) {Gen. Spec. 1};
  \node[ov text] at (308.83,299.5) {Gen. Spec. 2};
  \node[ov text] at (335.00,319.5) {...};
  \node[ov text] at (446.66,279.5) {Isom. Proof 1};
  \node[ov text] at (446.66,299.5) {Isom. Proof 2};
  \node[ov text] at (475.00,319.5) {...};
  \node[ov text] at (239.83,340) {SPEC\_GEN};
  \node[ov text] at (382.48,340) {SPEC\_ISO};
  \node[ov text] at (514.83,340) {IMPL\_GEN};
  \node[ov text] at (639.83,340) {PROOF\_GEN};
  \node[ov text, rotate=90, font=\ovfont{9}] at (152.95,192.45) {CLEVER};

  \node[ov label] at (269.16,170.5) {Simple};
  \node[ov label] at (409.16,170.5) {Simple};
  \node[ov label] at (268.05,225.5) {Guided};
  \node[ov label] at (408.05,225.5) {Guided};
  \node[ov label] at (263.05,290.5) {Multiple};
  \node[ov label] at (404.05,290.5) {Multiple};
  \node[ov small] at (535.00,242.5) {(Simple)};
  \node[ov small] at (666.00,241.5) {(Simple)};
  \node[ov small] at (536.00,296.5) {(Guided)};
  \node[ov small] at (665.00,298.5) {(Guided)};
  \foreach \x/\y/\t in {533.92/169.5/Gr.-T., 663.92/169.5/Gr.-T., 537.45/224.5/Gen.,
                        667.45/214.5/Gen., 538.45/278.5/Gen., 667.45/269.5/Gen.} {
    \node[ov arrow] at (\x+4.19,\y) {\char212};
    \node[ov label] at (\x+10.88,\y) {\t};
  }
\end{tikzpicture}%


==> tables/results_impl_matrix.tex <==
\mainfloatbegin
  \moveups
  \caption{Implementation certification, one attempt per entry and run; cells give count (\%). \emph{Top}: against the reference specification (\clever{}'s protocol), one run per stack; \emph{Certified} is \proofgen{} \flagOK{} against \probspec{}, and end-to-end success also requires a \emph{Valid} or \emph{Accepted} Simple or Guided specification, \emph{Accepted} being \clever{}'s end-to-end criterion (1/161 in the original evaluation; with Claude's Multiple run, \emph{Valid} 102 and 68, \emph{Accepted} 59 and 59). \emph{Bottom}: against each stack's own generated specification, per \specgen{} chain (\emph{Any}: either chain); proofs are independently recompiled and make no claim on the specification's validity, and end-to-end success requires a \emph{Valid} or \emph{Accepted} specification from the same chain, whose isomorphism transfers the proof to \probspec{}. Terms as in Sections~\ref{sec:results-spec} and~\ref{sec:results-impl}.}
  \label{tab:results-impl-matrix}
  \label{tab:results-e2e-matrix}
  \moveups
  \centering
  \footnotesize
  \setlength{\tabcolsep}{3.5pt}
  \begin{tabular}{@{}l r r r r r r@{}}
    \toprule
    \emph{count (\%)} & \multicolumn{2}{c}{Certified} & \multicolumn{2}{c}{End-to-end Valid} & \multicolumn{2}{c}{End-to-end Accepted} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(l){6-7}
    Stack & /161 & $C_\mathrm{gt}$ /78 & /161 & $C_\mathrm{gt}$ /78 & /161 & $C_\mathrm{gt}$ /78 \\
    \midrule
    Claude Code + Opus~4.6 & 104~{\scriptsize(64.6\%)} & 70~{\scriptsize(89.7\%)} & 101~{\scriptsize(62.7\%)} & 67~{\scriptsize(85.9\%)} & 55~{\scriptsize(34.2\%)} & 55~{\scriptsize(70.5\%)} \\
    Codex CLI + GPT-5.4 & 105~{\scriptsize(65.2\%)} & 72~{\scriptsize(92.3\%)} & 100~{\scriptsize(62.1\%)} & 68~{\scriptsize(87.2\%)} & 56~{\scriptsize(34.8\%)} & 55~{\scriptsize(70.5\%)} \\
    OpenHands + Kimi K2.5 & 77~{\scriptsize(47.8\%)} & 53~{\scriptsize(67.9\%)} & 67~{\scriptsize(41.6\%)} & 44~{\scriptsize(56.4\%)} & 35~{\scriptsize(21.7\%)} & 35~{\scriptsize(44.9\%)} \\
    \midrule
    \textbf{Union} (any stack) & 109~{\scriptsize(67.7\%)} & 74~{\scriptsize(94.9\%)} & 108~{\scriptsize(67.1\%)} & 73~{\scriptsize(93.6\%)} & 63~{\scriptsize(39.1\%)} & 62~{\scriptsize(79.5\%)} \\
    \bottomrule
  \end{tabular}

  \vspace{3mm}
  {
  \footnotesize
  \setlength{\tabcolsep}{3.5pt}
  \begin{tabular}{@{}c l r r r r r r@{}}
    \toprule
    \multicolumn{2}{@{}l}{\emph{count (\%)}} & \multicolumn{2}{c}{Certified} & \multicolumn{2}{c}{End-to-end Valid} & \multicolumn{2}{c}{End-to-end Accepted} \\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(l){7-8}
    Stack & Chain & /161 & $C_\mathrm{gen}$ /157 & /161 & $C_\mathrm{gen}$ /157 & /161 & $C_\mathrm{gen}$ /157 \\
    \midrule
    \multirow{3}{*}{\begin{tabular}{@{}c@{}}\textbf{Claude Code}\\+\\\textbf{Opus~4.6}\end{tabular}} & Simple chain & 144~{\scriptsize(89.4\%)} & 144~{\scriptsize(91.7\%)} & 135~{\scriptsize(83.9\%)} & 135~{\scriptsize(86.0\%)} & 56~{\scriptsize(34.8\%)} & 56~{\scriptsize(35.7\%)} \\
     & Guided chain & 148~{\scriptsize(91.9\%)} & 148~{\scriptsize(94.3\%)} & 145~{\scriptsize(90.1\%)} & 145~{\scriptsize(92.4\%)} & 56~{\scriptsize(34.8\%)} & 56~{\scriptsize(35.7\%)} \\
     & {\itshape Any} & {\itshape 154~{\scriptsize(95.7\%)}} & {\itshape 154~{\scriptsize(98.1\%)}} & {\itshape 151~{\scriptsize(93.8\%)}} & {\itshape 151~{\scriptsize(96.2\%)}} & {\itshape 60~{\scriptsize(37.3\%)}} & {\itshape 60~{\scriptsize(38.2\%)}} \\
    \midrule
    \multirow{3}{*}{\begin{tabular}{@{}c@{}}\textbf{Codex CLI}\\+\\\textbf{GPT-5.4}\end{tabular}} & Simple chain & 142~{\scriptsize(88.2\%)} & 141~{\scriptsize(89.8\%)} & 125~{\scriptsize(77.6\%)} & 125~{\scriptsize(79.6\%)} & 48~{\scriptsize(29.8\%)} & 48~{\scriptsize(30.6\%)} \\
     & Guided chain & 142~{\scriptsize(88.2\%)} & 141~{\scriptsize(89.8\%)} & 128~{\scriptsize(79.5\%)} & 127~{\scriptsize(80.9\%)} & 54~{\scriptsize(33.5\%)} & 54~{\scriptsize(34.4\%)} \\
     & {\itshape Any} & {\itshape 155~{\scriptsize(96.3\%)}} & {\itshape 153~{\scriptsize(97.5\%)}} & {\itshape 143~{\scriptsize(88.8\%)}} & {\itshape 142~{\scriptsize(90.4\%)}} & {\itshape 57~{\scriptsize(35.4\%)}} & {\itshape 57~{\scriptsize(36.3\%)}} \\
    \midrule
    \multirow{3}{*}{\begin{tabular}{@{}c@{}}\textbf{OpenHands}\\+\\\textbf{Kimi K2.5}\end{tabular}} & Simple chain & 123~{\scriptsize(76.4\%)} & 123~{\scriptsize(78.3\%)} & 98~{\scriptsize(60.9\%)} & 98~{\scriptsize(62.4\%)} & 30~{\scriptsize(18.6\%)} & 30~{\scriptsize(19.1\%)} \\
     & Guided chain & 119~{\scriptsize(73.9\%)} & 119~{\scriptsize(75.8\%)} & 95~{\scriptsize(59.0\%)} & 95~{\scriptsize(60.5\%)} & 34~{\scriptsize(21.1\%)} & 34~{\scriptsize(21.7\%)} \\
     & {\itshape Any} & {\itshape 140~{\scriptsize(87.0\%)}} & {\itshape 140~{\scriptsize(89.2\%)}} & {\itshape 118~{\scriptsize(73.3\%)}} & {\itshape 118~{\scriptsize(75.2\%)}} & {\itshape 38~{\scriptsize(23.6\%)}} & {\itshape 38~{\scriptsize(24.2\%)}} \\
    \midrule
    \multicolumn{2}{@{}l}{\textbf{Union} (any stack, any chain) }& 158~{\scriptsize(98.1\%)} & 156~{\scriptsize(99.4\%)} & 156~{\scriptsize(96.9\%)} & 155~{\scriptsize(98.7\%)} & 65~{\scriptsize(40.4\%)} & 65~{\scriptsize(41.4\%)} \\
    \bottomrule
  \end{tabular}
  }
  \moveup
  \moveup
\mainfloatend


==> tables/results_spec_matrix.tex <==
\mainfloatbegin
  \moveups
  \caption{Specification certification: \speciso{} outcomes on each stack's \specgen{} output, one attempt per entry and run; cells give count (\%). \emph{Valid}, \emph{Accepted}, and $C_\mathrm{spec}$ as in Section~\ref{sec:results-spec}; \emph{Any}: at least one run succeeds (S, G, M: Simple, Guided, Multiple). Multiple: Claude only, on the 105 entries without a Guided \flagOK{} (24 in $C_\mathrm{spec}$), succeeding if any of up to four candidates does. Claude's Any (S+G+M) row matches its merged annotation: all entries but the 2 \flagFAIL{} are \emph{Valid}, and exactly the 65 \flagOK{} entries are \emph{Accepted}. Union: any stack, any run.}
  \moveups
  \label{tab:results-spec-matrix}
  \centering
  \footnotesize
  \setlength{\tabcolsep}{5pt}
  \begin{tabular}{@{}c l r r r r@{}}
    \toprule
    \multicolumn{2}{@{}l}{\emph{count (\%)}} & \multicolumn{2}{c}{Valid} & \multicolumn{2}{c}{Accepted} \\
    \cmidrule(lr){3-4} \cmidrule(l){5-6}
    Stack & Run & /161 & $C_\mathrm{spec}$ /80 & /161 & $C_\mathrm{spec}$ /80 \\
    \midrule
    \multirow{5}{*}{\begin{tabular}{@{}c@{}}\textbf{Claude Code}\\+\\\textbf{Opus~4.6}\end{tabular}} & Simple & 147~{\scriptsize(91.3\%)} & 70~{\scriptsize(87.5\%)} & 59~{\scriptsize(36.6\%)} & 58~{\scriptsize(72.5\%)} \\
     & Guided & 157~{\scriptsize(97.5\%)} & 76~{\scriptsize(95.0\%)} & 56~{\scriptsize(34.8\%)} & 56~{\scriptsize(70.0\%)} \\
     & {\itshape Any (S+G)} & {\itshape 158~{\scriptsize(98.1\%)}} & {\itshape 77~{\scriptsize(96.3\%)}} & {\itshape 62~{\scriptsize(38.5\%)}} & {\itshape 61~{\scriptsize(76.3\%)}} \\
     & Multiple & 101\phantom{~{\scriptsize(00.0\%)}} & 21\phantom{~{\scriptsize(00.0\%)}} & 11\phantom{~{\scriptsize(00.0\%)}} & 9\phantom{~{\scriptsize(00.0\%)}} \\
     & {\itshape Any (S+G+M)} & {\itshape 159~{\scriptsize(98.8\%)}} & {\itshape 78~{\scriptsize(97.5\%)}} & {\itshape 67~{\scriptsize(41.6\%)}} & {\itshape 65~{\scriptsize(81.3\%)}} \\
    \midrule
    \multirow{3}{*}{\begin{tabular}{@{}c@{}}\textbf{Codex CLI}\\+\\\textbf{GPT-5.4}\end{tabular}} & Simple & 136~{\scriptsize(84.5\%)} & 65~{\scriptsize(81.3\%)} & 49~{\scriptsize(30.4\%)} & 48~{\scriptsize(60.0\%)} \\
     & Guided & 140~{\scriptsize(87.0\%)} & 67~{\scriptsize(83.8\%)} & 56~{\scriptsize(34.8\%)} & 55~{\scriptsize(68.8\%)} \\
     & {\itshape Any} & {\itshape 150~{\scriptsize(93.2\%)}} & {\itshape 73~{\scriptsize(91.3\%)}} & {\itshape 60~{\scriptsize(37.3\%)}} & {\itshape 58~{\scriptsize(72.5\%)}} \\
    \midrule
    \multirow{3}{*}{\begin{tabular}{@{}c@{}}\textbf{OpenHands}\\+\\\textbf{Kimi K2.5}\end{tabular}} & Simple & 121~{\scriptsize(75.2\%)} & 52~{\scriptsize(65.0\%)} & 34~{\scriptsize(21.1\%)} & 33~{\scriptsize(41.3\%)} \\
     & Guided & 123~{\scriptsize(76.4\%)} & 57~{\scriptsize(71.3\%)} & 42~{\scriptsize(26.1\%)} & 41~{\scriptsize(51.3\%)} \\
     & {\itshape Any} & {\itshape 140~{\scriptsize(87.0\%)}} & {\itshape 63~{\scriptsize(78.8\%)}} & {\itshape 46~{\scriptsize(28.6\%)}} & {\itshape 44~{\scriptsize(55.0\%)}} \\
    \midrule
    \multicolumn{2}{@{}l}{\textbf{Union} (any stack, any run) }& 160~{\scriptsize(99.4\%)} & 79~{\scriptsize(98.8\%)} & 73~{\scriptsize(45.3\%)} & 68~{\scriptsize(85.0\%)} \\
    \bottomrule
  \end{tabular}
  \moveup
\mainfloatend

